A framework for the architecture of exoplanetary systems. I. Four classes of planetary system architecture

We present a novel, model-independent framework for studying the architecture of an exoplanetary system at the system level. This framework allows us to characterise, quantify, and classify the architecture of an individual planetary system. Our aim in this endeavour is to generate a systematic method to study the arrangement and distribution of various planetary quantities within a single planetary system. We propose that the space of planetary system architectures be partitioned into four classes: similar, mixed, anti-ordered, and ordered. We applied our framework to observed and synthetic multi-planetary systems, thereby studying their architectures of mass, radius, density, core mass, and the core water mass fraction. We explored the relationships between a system's (mass) architecture and other properties. Our work suggests that: (a) similar architectures are the most common outcome of planet formation; (b) internal structure and composition of planets shows a strong link with their system architecture; (c) most systems inherit their mass architecture from their core mass architecture; (d) most planets that started inside the ice line and formed in-situ are found in systems with a similar architecture; and (e) most anti-ordered systems are expected to be rich in wet planets, while most observed mass ordered systems are expected to have many dry planets. We find, in good agreement with theory, that observations are generally biased towards the discovery of systems whose density architectures are similar, mixed, or anti-ordered. This study probes novel questions and new parameter spaces for understanding theory and observations. Future studies may utilise our framework to not only constrain the knowledge of individual planets, but also the multi-faceted architecture of an entire planetary system. We also speculate on the role of system architectures in hosting habitable worlds.

==> limits.tex <==
Consider a set $\mathcal{Q}$ of quantities $q$, i.e. $\mathcal{Q} = \{q_i\}$ where $q_i$ could be the mass, radius or other parameter of a planet, and the index $i \in [1,\nplanet]$ identifies a planet (with 1 being the innermost planet). We assume that all $q_i \ge 0$. The quantities $q_i$ are expressed as:
\begin{equation}
\label{eq:qi_decomposition_appendix}
	q_i = q' \ (1 \pm t_i).
\end{equation}
The quantities $q_i$ are decomposed around some value $q'$ such that all $t_i$ are minimized. $t_i$ measures the fractional difference (or tolerance) between $q'$ and $q_i$. Since all individual tolerances are a positive quantity, they will satisfy the following relation:
\begin{equation}
	0 \le t_i \le t.
\end{equation}

%------------------------------
\subsection{Mean}
Let us consider the mean of the quantities, $\bar{q_i}$:

\begin{equation}
\begin{split}
	\bar{q_i} 	&= \frac{Q}{\nplanet}  \ = \frac{\sum_i q_i}{\nplanet}\\
				&= \frac{q'}{\nplanet} \big(\nplanet \pm t_1 \pm t_2 \pm \dots  \pm t_\nplanet \big)
\end{split}
\end{equation}
The mean takes its maximum value only when all individual $t_i$'s take their maximum value and add up. This gives:
\begin{equation}
\begin{split}
	\max \bar{q_i} = q' \ \big(1 + t\big)
\end{split}
\end{equation}
Similarly, the minimum value of the mean is:
\begin{equation}
\begin{split}
\min \bar{q_i} = q' \ \big(1 - t\big)
\end{split}
\end{equation}

The extreme value of the mean occurs when all the individual quantities are extremized. However, in this scenario, since all quantities are equal, the \cvtext/ is identically 0.

%------------------------------
\subsection{Coefficient of Similarity}

We start with the definition of the \cstext/,
	\begin{equation}
		\cs (q) = \frac{1}{\nplanet - 1}  \ \sum_{i=1}^{i=\nplanet - 1} \  \Bigg(log \ \frac{q_{i+1}}{q_i} \ \Bigg).
	\end{equation}
Inserting eq. \ref{eq:qi_decomposition_appendix}, in the definition, we get:
\begin{equation}
	\cs (q) = \frac{1}{\nplanet - 1}  \ \sum_{i=1}^{i=\nplanet - 1} \  \Bigg(log \ \frac{1 \pm t_{i+1}}{1 \pm t_i} \ \Bigg).
\end{equation}
This formulation shows that the \cstext/ depends only on the fractional differences (tolerances) between $q_i$'s and not on their actual values. This is a desirable property. 
 
Next, we evaluate the $\max \cs$ as, 
\begin{equation}
\begin{split}
 \max \cs (q) &= \max \Bigg[ \frac{1}{\nplanet - 1}  \ \sum_{i=1}^{i=\nplanet - 1} \  \Bigg(log \ \frac{1 \pm t_{i+1}}{1 \pm t_i} \ \Bigg)  \Bigg],
 			\\&= \frac{1}{\nplanet - 1} \max \Bigg[ \sum_{i=1}^{i=\nplanet - 1} \  \Bigg(log \ \frac{1 \pm t_{i+1}}{1 \pm t_i} \ \Bigg) \Bigg],
 			\\&= \frac{1}{\nplanet - 1} \sum_{i=1}^{i=\nplanet - 1} \ log \   \max \Bigg[ \frac{1 \pm t_{i+1}}{1 \pm t_i} \Bigg].
\end{split}
\end{equation}
In the first step, we commuted the $\max$ operator with the fraction $(\nplanet - 1)^{-1}$ because we are interested in the maximum for a constant $\nplanet$.  Next, knowing that the maximum of a sum occurs at the sum of maximum summands and that $log$ is a monotonically increasing function, we further commute the $\max$ operator.

We observe,
\begin{equation}
	\max \Bigg[ \frac{1 \pm t_{i+1}}{1 \pm t_i} \Bigg] \quad \quad \text{when} \quad 
	\left\{
	\begin{array}{lr}
	\pm t_{i+1} &\rightarrow + t
	\\ 	
	\pm t_{i}	&\rightarrow - t
	\end{array}
	\right\}.
\end{equation}

This implies that
\begin{equation}
\label{eq:cslimit}
\begin{split}
	\max \ \cs (q) &= log \ \frac{1 + t}{1 - t},
	\\ 	
	\min \ \cs (q) &= - \max \ \cs = log \ \frac{1 - t}{1 + t},
\end{split}
\end{equation}
where the second equality can be similarly derived. Fig. \ref{fig:cscvlimits} shows the variation of $\max \ \cs$ as a function of tolerance $t$. We note that the limits of the \cstext/ do not depend on $\nplanet$, and we verified our results with numerical simulations. $\blacksquare$



%------------------------------
\subsection{Coefficient of Variation}

We start with the definition of the \cvtext/,
\begin{equation}
	\cv (q) = \frac{\sigma(q)}{\bar{q}}
\end{equation}
We note that the minimum value of the \cvtext/ is zero and it occurs when all $q_i$'s have equal value, thereby no variance. 

In the literature, we can find some derivations for the maximum value of the \cvtext/ \citep{Katsnelson1957,Sharma2010}. \cite{Katsnelson1957} show that the upper limit of the \cvtext/ is $\sqrt{\nplanet - 1}$ when all but one $q_i$ is zero. However, this limit is only a particular case of our formulation (specifically, $q_1 = q'$ and $q_{i \ne 1} = 0$). Here, we derive the limits for a more general scenario.

Consider, 
\begin{equation}
	\cv^2  = \frac{1}{\nplanet} \ \sum_{i=1}^{i=\nplanet} \ \bigg(\underbrace{1 - \frac{q_i}{\bar{q}}}_{= A} \bigg)^2.
\end{equation}
Here, we have squared the definition of $\cv$ and used the definition of the standard deviation $\sigma(q)$. As an aside, we note that the equation above shows that the \cvtext/ is zero when all $q_i = \bar{q}$, as noted before. We note that the maximum value of $\cv^2$ occurs when the term $A$ (in parenthesis) is maximized. Denoting $\sum_{i=1} q_i$ by $Q$, we consider the term in the parenthesis,
\begin{equation}
	A = 1 - \frac{\nplanet q_i}{Q} = \frac{Q - \nplanet q_i}{Q}.
\end{equation}

The condition for the general maxima of the \cvtext/, in our formulation, is when one of the quantity (say $q_1$ takes the largest possible value, while all others take the smallest possible value):
\begin{equation}
\begin{split}
	q_1 &= q' \ (1+t) \\
	q_{i \ne 1} &= q' \ (1-t).
\end{split}
\end{equation}
The mean in this scenario becomes (marked with $''$):
\begin{equation}
	\bar{q}'' = \frac{q'(1+t) + (n-1) \times q(1-t)}{\nplanet} = \frac{q'}{\nplanet} \bigg[ n(1-t) + 2t\bigg].
\end{equation}
The variance in this scenario becomes (marked with $''$):
\begin{equation}
	\sigma''^{2}  (q) = \frac{1}{\nplanet} \Biggl\{ \bigg[\underbrace{q'(1+t) - \bar{q}''}_{= \ 2q't \big(\frac{\nplanet-1}{\nplanet}\big)}\bigg]^2  + \ (\nplanet-1) \bigg[ \underbrace{q'(1-t) - \bar{q}''}_{= \ \frac{- 2 q' t}{\nplanet}} \bigg]^2     \Biggr\}.
\end{equation}
This gives, 
\begin{equation}
	\sigma'' (q) = \bigg(\frac{2 q' t}{\nplanet}\bigg) \sqrt{\nplanet - 1}.
\end{equation}

Finally, the general expression for the maximum value of the \cvtext/ becomes:
\begin{equation}
	\max \cv (q) = \frac{\sigma''(q)}{\bar{q}''} =  \frac{2t \ \sqrt{\nplanet - 1}}{n (1-t) + 2t}.
\end{equation}

\change{This expression recovers the particular case derived in literature when we set $t=1$. From this expression, we note that the upper limit of the \cvtext/ does not depend on the actual values of the quantities, but it depends on the number of quantities in the set $\mathcal{Q}$ and the maximum tolerance $t$. This new formulation allows us to extract the upper limit of the \cvtext/ for any set whose maximum tolerance $t$ is known. Interestingly, the above expression gives appropriate result when absurd inputs are considered. For example, when there are no planets in a system $\max \cv \big|_{\nplanet = 0} = \sqrt{-1}$ and when there is only one planet in a system $\max \cv \big|_{\nplanet = 1} = 0$. For a system of two planets the upper limit is exactly the fractional difference (or tolerance), i.e. $\max \cv \big|_{\nplanet = 2} = t$. }
	
Furthermore, varying over $\nplanet$, and assuming $t \in [0,1)$, allows us to derive the theoretical maximum possible value for the \cvtext/. This occurs at $\nplanet = \frac{2}{1 - t}$ and gives:
% 	\begin{equation}
% 	\label{eq:cvlimit}
% 		\max \cv (q) =  \frac{2 t \ \sqrt{\nplanet - 1}}{\nplanet (1-t) + 2 t}.
% 	\end{equation} 
	\begin{equation}
	\label{eq:cvlimit}
		\max \ \cv (q) \bigg|_{\nplanet = \frac{2}{1-t} } (q) = \frac{t}{\sqrt{1 - t^2}}.
	\end{equation}
Fig. \ref{fig:cscvlimits} shows the variation of the theoretical $\max \ \cv$ as a function of tolerance $t$.$\blacksquare$

==> table1_content.tex <==
\begin{tabular}{rclllllll}
\toprule
   Hostname & $n_\mathrm{planet}$ & $M_\star [M_\odot]$ & $R_\star [R_\odot]$ & $L_\star [L_\odot]$ & $T_\mathrm{eff} [K]$ &              [Fe/H] &         Age [Gyr] & Distance [pc] \\
\midrule
        Sun &                   8 &                 $1$ &                 $1$ &                 $1$ &              $5,772$ &                 $0$ &  $04.6 \pm \ 0.1$ &           $0$ \\
 Trappist-1 &                   7 &   $0.1 \pm \ 0.002$ &   $0.1 \pm \ 0.001$ &          $5.53e-04$ &    $2,566 \pm \ 026$ &  $+0.04 \pm \ 0.08$ &  $07.6 \pm \ 2.2$ &       $012.0$ \\
    TOI-178 &                   6 &    $0.7 \pm \ 0.03$ &    $0.7 \pm \ 0.01$ &   $0.1 \pm \ 01.08$ &    $4,316 \pm \ 070$ &  $-0.23 \pm \ 0.05$ &  $07.1 \pm \ 6.1$ &       $062.7$ \\
   HD 10180 &                   6 &    $1.1 \pm \ 0.05$ &    $1.1 \pm \ 0.04$ &   $1.5 \pm \ 00.02$ &    $5,911 \pm \ 019$ &  $+0.08 \pm \ 0.01$ &  $04.3 \pm \ 0.5$ &       $039.0$ \\
  HD 219134 &                   6 &    $0.8 \pm \ 0.03$ &   $0.8 \pm \ 0.005$ &   $0.3 \pm \ 00.01$ &    $4,700 \pm \ 020$ &  $+0.11 \pm \ 0.04$ &  $11.0 \pm \ 2.2$ &       $006.5$ \\
   HD 34445 &                   6 &    $1.1 \pm \ 0.02$ &    $1.4 \pm \ 0.08$ &   $2.0 \pm \ 01.11$ &    $5,836 \pm \ 044$ &  $+0.14 \pm \ 0.04$ &  $08.5 \pm \ 2.0$ &       $046.1$ \\
  Kepler-11 &                   6 &    $1.1 \pm \ 0.07$ &    $1.1 \pm \ 0.02$ &   $1.3 \pm \ 11.75$ &    $5,969 \pm \ 106$ &  $+0.01 \pm \ 0.13$ &  $02.4 \pm \ 2.5$ &       $645.6$ \\
  Kepler-20 &                   6 &    $0.9 \pm \ 0.05$ &    $0.9 \pm \ 0.02$ &   $0.6 \pm \ 28.25$ &    $5,438 \pm \ 087$ &  $+0.07 \pm \ 0.13$ &  $04.1 \pm \ 4.3$ &       $282.4$ \\
  Kepler-80 &                   6 &    $0.7 \pm \ 0.03$ &    $0.7 \pm \ 0.01$ &   $0.2 \pm \ 92.90$ &    $4,453 \pm \ 077$ &  $+0.13 \pm \ 0.11$ &  $10.7 \pm \ 6.7$ &       $367.6$ \\
     K2-138 &                   6 &    $0.9 \pm \ 0.02$ &    $0.9 \pm \ 0.03$ &   $0.5 \pm \ 00.02$ &    $5,356 \pm \ 042$ &  $+0.14 \pm \ 0.04$ &  $02.8 \pm \ 3.8$ &       $202.6$ \\
\bottomrule
\end{tabular}



==> table2_content.tex <==
\begin{tabular}{rcccc}
\toprule
     Hostname & Multiplicity & $C_{S}(M)$ & $C_{V}(M)$ & Architecture Type \\
\midrule
 Solar System &          $8$ &    $+0.36$ &       1.85 &           Ordered \\
   Trappist-1 &          $7$ &    $-0.10$ &       0.45 &           Similar \\
      TOI-178 &          $6$ &    $+0.08$ &       0.46 &           Similar \\
     HD 10180 &          $6$ &    $+0.14$ &       0.66 &           Similar \\
    HD 219134 &          $6$ &    $+0.27$ &       1.49 &           Ordered \\
     HD 34445 &          $6$ &    $+0.17$ &       0.84 &           Similar \\
    Kepler-11 &          $6$ &    $+0.22$ &       1.03 &           Ordered \\
    Kepler-20 &          $6$ &    $+0.00$ &       0.44 &           Similar \\
    Kepler-80 &          $6$ &    $-0.00$ &       0.19 &           Similar \\
       K2-138 &          $6$ &    $+0.03$ &       0.61 &           Similar \\
       55 Cnc &          $5$ &    $+0.52$ &       1.37 &           Ordered \\
     GJ 667 C &          $5$ &    $-0.02$ &       0.29 &           Similar \\
    HD 158259 &          $5$ &    $+0.11$ &       0.29 &           Similar \\
     HD 40307 &          $5$ &    $+0.07$ &       0.33 &           Similar \\
   Kepler-102 &          $5$ &    $+0.02$ &       0.41 &           Similar \\
    Kepler-33 &          $5$ &    $+0.46$ &       0.67 &           Ordered \\
    Kepler-62 &          $5$ &    $+0.15$ &       0.68 &           Similar \\
     HD 20781 &          $4$ &    $+0.29$ &       0.59 &           Ordered \\
      TOI-561 &          $4$ &    $+0.33$ &       0.64 &           Ordered \\
       DMPP-1 &          $4$ &    $+0.29$ &       0.81 &           Ordered \\
      GJ 3293 &          $4$ &    $+0.27$ &       0.62 &           Ordered \\
     GJ 676 A &          $4$ &    $+0.90$ &       0.99 &           Ordered \\
       GJ 876 &          $4$ &    $+0.12$ &       1.20 &             Mixed \\
    HD 141399 &          $4$ &    $+0.06$ &       0.40 &           Similar \\
    HD 160691 &          $4$ &    $+0.63$ &       0.82 &           Ordered \\
     HD 20794 &          $4$ &    $+0.08$ &       0.25 &           Similar \\
    HD 215152 &          $4$ &    $+0.07$ &       0.23 &           Similar \\
      HR 8799 &          $4$ &    $-0.07$ &       0.17 &           Similar \\
       K2-266 &          $4$ &    $+0.03$ &       0.60 &           Similar \\
       K2-285 &          $4$ &    $+0.01$ &       0.31 &           Similar \\
    Kepler-89 &          $4$ &    $+0.17$ &       0.91 &             Mixed \\
   Kepler-106 &          $4$ &    $+0.11$ &       0.26 &           Similar \\
   Kepler-107 &          $4$ &    $+0.13$ &       0.42 &           Similar \\
   Kepler-223 &          $4$ &    $-0.06$ &       0.22 &           Similar \\
   Kepler-411 &          $4$ &    $-0.08$ &       0.34 &           Similar \\
    Kepler-48 &          $4$ &    $+0.74$ &       1.64 &           Ordered \\
    Kepler-65 &          $4$ &    $+0.68$ &       1.63 &           Ordered \\
    Kepler-79 &          $4$ &    $-0.10$ &       0.24 &           Similar \\
      WASP-47 &          $4$ &    $+0.59$ &       0.95 &           Ordered \\
      tau Cet &          $4$ &    $+0.12$ &       0.37 &           Similar \\
    HD 164922 &          $4$ &    $+0.49$ &       1.29 &           Ordered \\
\bottomrule
\end{tabular}


